Focused Model-Learning and Planning for Non-Gaussian Continuous State-Action Systems

We introduce a framework for model learning and planning in stochastic domains with continuous state and action spaces and non-Gaussian transition models. It is efficient because (1) local models are estimated only when the planner requires them; (2) the planner focuses on the most relevant states to the current planning problem; and (3) the planner focuses on the most informative and/or high-value actions. Our theoretical analysis shows the validity and asymptotic optimality of the proposed approach. Empirically, we demonstrate the effectiveness of our algorithm on a simulated multi-modal pushing problem.

==> planning.tex <==

\subsection{Planning in \ALGNAME}
\label{ssec:plan}
At the highest level, \ALGNAME  
operates in a loop, in which it samples a
discrete set of states and attempts to solve the discrete-state,
continuous-action MDP induced by that sampled state set. The input to
\ALGNAME includes the starting state $s_0$, the goal region $\mathcal G$,
the continuous state space $S$, the function handle that computes the
next state density $p_{s'|s,a}$, and the minimum number of states,
$N_{\min}$, to sample at each iteration.  It may be that more than
$N_{\min}$ states are sampled, because sampling must continue until at
least one goal state is included in the resulting set $\tilde S$. If
the value of the resulting policy computed from RTDP is satisfactory,
it is returned, otherwise, additional state samples are added and the
process is repeated. The user can define the function
$\textsc{callback}$ to specify the desired termination condition on
the resulting policy.

\begin{algorithm}[t]
\scriptsize
\caption{\ALGNAME}
\label{alg:zw}
\begin{algorithmic}[1]
\Function{\ALGNAME}{$s_0, \mathcal G, S, p_{s'|s,a}, N_{\min}$}
\State $\tilde S\gets \{s_0\}$
\Loop
\State $\tilde S \gets \textsc{SampleStates}(N_{\min},\tilde S, \mathcal G, S, p_{s'|s,a})$
\State $\pi, V = \textsc{RTDP}(s_{0},\mathcal G, \tilde S, p_{s'|s,a})$
\EndLoop
\State \textbf{until} \textsc{callback}($\pi$, $V$)
\State \Return $\pi, V$
\EndFunction
\Statex
\Function{callback}{$\pi,V$}
\LineComment User-defined function to judge if $\pi, V$ are good enough to return. 
\EndFunction
\end{algorithmic}
\end{algorithm}



